Orientation Aware Weapons Detection In Visual Data : A Benchmark Dataset

Automatic detection of weapons is significant for improving security and well being of individuals, nonetheless, it is a difficult task due to large variety of size, shape and appearance of weapons. View point variations and occlusion also are reasons which makes this task more difficult. Further, the current object detection algorithms process rectangular areas, however a slender and long rifle may really cover just a little portion of area and the rest may contain unessential details. To overcome these problem, we propose a CNN architecture for Orientation Aware Weapons Detection, which provides oriented bounding box with improved weapons detection performance. The proposed model provides orientation not only using angle as classification problem by dividing angle into eight classes but also angle as regression problem. For training our model for weapon detection a new dataset comprising of total 6400 weapons images is gathered from the web and then manually annotated with position oriented bounding boxes. Our dataset provides not only oriented bounding box as ground truth but also horizontal bounding box. We also provide our dataset in multiple formats of modern object detectors for further research in this area. The proposed model is evaluated on this dataset, and the comparative analysis with off-the shelf object detectors yields superior performance of proposed model, measured with standard evaluation strategies. The dataset and the model implementation are made publicly available at this link: https://bit.ly/2TyZICF.

==> cas-refs <==
@inproceedings{moian2018walking,
  title={WALKING THE ROAD OF EDUCATION UNDER GUN THREAT: CASE OF THE USA},
  author={MOIAN, Daniela and STR{\^A}MBEANU, Oana},
  booktitle={THE 20 th STUDENTS’INTERNATIONAL CONFERENCE},
  pages={49},
  year={2018}
}
@article{morris2018mass,
  title={Mass shootings in the US: There have been 1,624 in 1,870 days},
  author={Morris, Sam},
  journal={The Guardian},
  year={2018}
}
@misc{Texas,
  author = {Jennifer Calfas},
  title = {{Texas Was the 22nd School Shooting This Year}},
  howpublished = "\url{https://time.com/5282496/santa-fe-high-school-shooting-2018/}",
  year = {2018}, 
  note = "[Online; accessed 13-August-2020]"
}
@article{nunes2012united,
  title={United Nations Office on Drugs and Crime (UNODC). Global Study on Homicide: Trends, Context, Data. Vienna: UNODC; 2011},
  author={Nunes, Everardo Duarte},
  journal={Ci{\^e}ncia \& Sa{\'u}de Coletiva},
  volume={17},
  pages={3447--3449},
  year={2012},
  publisher={SciELO Public Health}
}
@article{planty2013firearm,
  title={Firearm Violence, 1993-2011 (NCJ 241730)},
  author={Planty, Michael and Truman, JL},
  journal={Special report prepared by the Bureau of Justice Statistics. Washington, DC},
  year={2013}
}
@misc{BBC,
  author = {BBC},
  title = {{America's gun culture in charts}},
  howpublished = "\url{https://www.bbc.com/news/world-us-canada-41488081}",
  year = {2019}, 
  note = "[Online; accessed 13-August-2020]"
}
@misc{NYT,
  author = { The New York Times},
  title = {{Opinion, Restore funding for gun violence research }},
  howpublished = "\url{https://www.nytimes.com/2018/11/06/ opinion/letters/gun violence-research.html}",
  year = {2018}, 
  note = "[Online; accessed 13-August-2020]"
}
@article{jaffe2018gun,
  title={Gun violence research in the USA: the CDC's impasse},
  author={Jaffe, Susan},
  journal={The Lancet},
  volume={391},
  number={10139},
  pages={2487--2488},
  year={2018},
  publisher={Elsevier}
}
@article{velastin2006motion,
  title={A motion-based image processing system for detecting potentially dangerous situations in underground railway stations},
  author={Velastin, Sergio A and Boghossian, Boghos A and Vicencio-Silva, Maria Alicia},
  journal={Transportation Research Part C: Emerging Technologies},
  volume={14},
  number={2},
  pages={96--113},
  year={2006},
  publisher={Elsevier}
}
@article{ainsworth2002buyer,
  title={Buyer beware},
  author={Ainsworth, Trevor},
  journal={Security Oz},
  volume={19},
  pages={18--26},
  year={2002}
}
@inproceedings{liu2016ssd,
  title={Ssd: Single shot multibox detector},
  author={Liu, Wei and Anguelov, Dragomir and Erhan, Dumitru and Szegedy, Christian and Reed, Scott and Fu, Cheng-Yang and Berg, Alexander C},
  booktitle={European conference on computer vision},
  pages={21--37},
  year={2016},
  organization={Springer}
}
@inproceedings{ren2015faster,
  title={Faster r-cnn: Towards real-time object detection with region proposal networks},
  author={Ren, Shaoqing and He, Kaiming and Girshick, Ross and Sun, Jian},
  booktitle={Advances in neural information processing systems},
  pages={91--99},
  year={2015}
}
@inproceedings{redmon2016you,
  title={You only look once: Unified, real-time object detection},
  author={Redmon, Joseph and Divvala, Santosh and Girshick, Ross and Farhadi, Ali},
  booktitle={Proceedings of the IEEE conference on computer vision and pattern recognition},
  pages={779--788},
  year={2016}
}
@article{hu2018sinet,
  title={SINet: A scale-insensitive convolutional neural network for fast vehicle detection},
  author={Hu, Xiaowei and Xu, Xuemiao and Xiao, Yongjie and Chen, Hao and He, Shengfeng and Qin, Jing and Heng, Pheng-Ann},
  journal={IEEE transactions on intelligent transportation systems},
  volume={20},
  number={3},
  pages={1010--1019},
  year={2018},
  publisher={IEEE}
}
@article{li2017scale,
  title={Scale-aware fast R-CNN for pedestrian detection},
  author={Li, Jianan and Liang, Xiaodan and Shen, ShengMei and Xu, Tingfa and Feng, Jiashi and Yan, Shuicheng},
  journal={IEEE transactions on Multimedia},
  volume={20},
  number={4},
  pages={985--996},
  year={2017},
  publisher={IEEE}
}
@inproceedings{li2017perceptual,
  title={Perceptual generative adversarial networks for small object detection},
  author={Li, Jianan and Liang, Xiaodan and Wei, Yunchao and Xu, Tingfa and Feng, Jiashi and Yan, Shuicheng},
  booktitle={Proceedings of the IEEE conference on computer vision and pattern recognition},
  pages={1222--1230},
  year={2017}
}
@article{liu2019towards,
  title={Towards accurate tiny vehicle detection in complex scenes},
  author={Liu, Wei and Liao, Shengcai and Hu, Weidong},
  journal={Neurocomputing},
  volume={347},
  pages={24--33},
  year={2019},
  publisher={Elsevier}
}
@inproceedings{zhang2016faster,
  title={Is faster R-CNN doing well for pedestrian detection?},
  author={Zhang, Liliang and Lin, Liang and Liang, Xiaodan and He, Kaiming},
  booktitle={European conference on computer vision},
  pages={443--457},
  year={2016},
  organization={Springer}
}
@inproceedings{zhou2017oriented,
  title={Oriented response networks},
  author={Zhou, Yanzhao and Ye, Qixiang and Qiu, Qiang and Jiao, Jianbin},
  booktitle={Proceedings of the IEEE Conference on Computer Vision and Pattern Recognition},
  pages={519--528},
  year={2017}
}
@inproceedings{azimi2018towards,
  title={Towards multi-class object detection in unconstrained remote sensing imagery},
  author={Azimi, Seyed Majid and Vig, Eleonora and Bahmanyar, Reza and K{\"o}rner, Marco and Reinartz, Peter},
  booktitle={Asian Conference on Computer Vision},
  pages={150--165},
  year={2018},
  organization={Springer}
}
@article{ma2018arbitrary,
  title={Arbitrary-oriented scene text detection via rotation proposals},
  author={Ma, Jianqi and Shao, Weiyuan and Ye, Hao and Wang, Li and Wang, Hong and Zheng, Yingbin and Xue, Xiangyang},
  journal={IEEE Transactions on Multimedia},
  volume={20},
  number={11},
  pages={3111--3122},
  year={2018},
  publisher={IEEE}
}
@inproceedings{deng2009imagenet,
  title={Imagenet: A large-scale hierarchical image database},
  author={Deng, Jia and Dong, Wei and Socher, Richard and Li, Li-Jia and Li, Kai and Fei-Fei, Li},
  booktitle={2009 IEEE conference on computer vision and pattern recognition},
  pages={248--255},
  year={2009},
  organization={Ieee}
}
@article{olmos2018automatic,
  title={Automatic handgun detection alarm in videos using deep learning},
  author={Olmos, Roberto and Tabik, Siham and Herrera, Francisco},
  journal={Neurocomputing},
  volume={275},
  pages={66--72},
  year={2018},
  publisher={Elsevier}
}
@inproceedings{girshick2014rich,
  title={Rich feature hierarchies for accurate object detection and semantic segmentation},
  author={Girshick, Ross and Donahue, Jeff and Darrell, Trevor and Malik, Jitendra},
  booktitle={Proceedings of the IEEE conference on computer vision and pattern recognition},
  pages={580--587},
  year={2014}
}
@inproceedings{redmon2017yolo9000,
  title={YOLO9000: better, faster, stronger},
  author={Redmon, Joseph and Farhadi, Ali},
  booktitle={Proceedings of the IEEE conference on computer vision and pattern recognition},
  pages={7263--7271},
  year={2017}
}
@inproceedings{dai2016r,
  title={R-fcn: Object detection via region-based fully convolutional networks},
  author={Dai, Jifeng and Li, Yi and He, Kaiming and Sun, Jian},
  booktitle={Advances in neural information processing systems},
  pages={379--387},
  year={2016}
}
@article{akcay2018using,
  title={Using deep convolutional neural network architectures for object classification and detection within x-ray baggage security imagery},
  author={Akcay, Samet and Kundegorski, Mikolaj E and Willcocks, Chris G and Breckon, Toby P},
  journal={IEEE transactions on information forensics and security},
  volume={13},
  number={9},
  pages={2203--2215},
  year={2018},
  publisher={IEEE}
}
@article{redmon2018yolov3,
  title={Yolov3: An incremental improvement},
  author={Redmon, Joseph and Farhadi, Ali},
  journal={arXiv preprint arXiv:1804.02767},
  year={2018}
}
@article{han2015deep,
  title={Deep compression: Compressing deep neural networks with pruning, trained quantization and huffman coding},
  author={Han, Song and Mao, Huizi and Dally, William J},
  journal={arXiv preprint arXiv:1510.00149},
  year={2015}
}
@article{fu2017dssd,
  title={Dssd: Deconvolutional single shot detector},
  author={Fu, Cheng-Yang and Liu, Wei and Ranga, Ananth and Tyagi, Ambrish and Berg, Alexander C},
  journal={arXiv preprint arXiv:1701.06659},
  year={2017}
}
@inproceedings{hu2017finding,
  title={Finding tiny faces},
  author={Hu, Peiyun and Ramanan, Deva},
  booktitle={Proceedings of the IEEE conference on computer vision and pattern recognition},
  pages={951--959},
  year={2017}
}
@article{grega2016automated,
  title={Automated detection of firearms and knives in a CCTV image},
  author={Grega, Micha{\l} and Matiola{\'n}ski, Andrzej and Guzik, Piotr and Leszczuk, Miko{\l}aj},
  journal={Sensors},
  volume={16},
  number={1},
  pages={47},
  year={2016},
  publisher={Multidisciplinary Digital Publishing Institute}
}
@inproceedings{lin2017focal,
  title={Focal loss for dense object detection},
  author={Lin, Tsung-Yi and Goyal, Priya and Girshick, Ross and He, Kaiming and Doll{\'a}r, Piotr},
  booktitle={Proceedings of the IEEE international conference on computer vision},
  pages={2980--2988},
  year={2017}
}

@article{tiwari2015computer,
  title={A computer vision based framework for visual gun detection using harris interest point detector},
  author={Tiwari, Rohit Kumar and Verma, Gyanendra K},
  journal={Procedia Computer Science},
  volume={54},
  pages={703--712},
  year={2015},
  publisher={Elsevier}
}
@inproceedings{harris1988combined,
  title={A combined corner and edge detector.},
  author={Harris, Christopher G and Stephens, Mike and others},
  booktitle={Alvey vision conference},
  volume={15},
  number={50},
  pages={10--5244},
  year={1988},
  organization={Citeseer}
}
@inproceedings{alahi2012freak,
  title={Freak: Fast retina keypoint},
  author={Alahi, Alexandre and Ortiz, Raphael and Vandergheynst, Pierre},
  booktitle={2012 IEEE Conference on Computer Vision and Pattern Recognition},
  pages={510--517},
  year={2012},
  organization={Ieee}
}
@inproceedings{liu2018structure,
  title={Structure inference net: Object detection using scene-level context and instance-level relationships},
  author={Liu, Yong and Wang, Ruiping and Shan, Shiguang and Chen, Xilin},
  booktitle={Proceedings of the IEEE conference on computer vision and pattern recognition},
  pages={6985--6994},
  year={2018}
}
@inproceedings{chen2018context,
  title={Context refinement for object detection},
  author={Chen, Zhe and Huang, Shaoli and Tao, Dacheng},
  booktitle={Proceedings of the European Conference on Computer Vision (ECCV)},
  pages={71--86},
  year={2018}
}
@inproceedings{huang2017speed,
  title={Speed/accuracy trade-offs for modern convolutional object detectors},
  author={Huang, Jonathan and Rathod, Vivek and Sun, Chen and Zhu, Menglong and Korattikara, Anoop and Fathi, Alireza and Fischer, Ian and Wojna, Zbigniew and Song, Yang and Guadarrama, Sergio and others},
  booktitle={Proceedings of the IEEE conference on computer vision and pattern recognition},
  pages={7310--7311},
  year={2017}
}
@article{uijlings2013selective,
  title={Selective search for object recognition},
  author={Uijlings, Jasper RR and Van De Sande, Koen EA and Gevers, Theo and Smeulders, Arnold WM},
  journal={International journal of computer vision},
  volume={104},
  number={2},
  pages={154--171},
  year={2013},
  publisher={Springer}
}
@article{furey2000support,
  title={Support vector machine classification and validation of cancer tissue samples using microarray expression data},
  author={Furey, Terrence S and Cristianini, Nello and Duffy, Nigel and Bednarski, David W and Schummer, Michel and Haussler, David},
  journal={Bioinformatics},
  volume={16},
  number={10},
  pages={906--914},
  year={2000},
  publisher={Oxford University Press}
}
@inproceedings{lin2017feature,
  title={Feature pyramid networks for object detection},
  author={Lin, Tsung-Yi and Doll{\'a}r, Piotr and Girshick, Ross and He, Kaiming and Hariharan, Bharath and Belongie, Serge},
  booktitle={Proceedings of the IEEE conference on computer vision and pattern recognition},
  pages={2117--2125},
  year={2017}
}
@inproceedings{he2017mask,
  title={Mask r-cnn},
  author={He, Kaiming and Gkioxari, Georgia and Doll{\'a}r, Piotr and Girshick, Ross},
  booktitle={Proceedings of the IEEE international conference on computer vision},
  pages={2961--2969},
  year={2017}
}











@article{swanson2015guns,
  title={Guns, impulsive angry behavior, and mental disorders: Results from the National Comorbidity Survey Replication (NCS-R)},
  author={Swanson, Jeffrey W and Sampson, Nancy A and Petukhova, Maria V and Zaslavsky, Alan M and Appelbaum, Paul S and Swartz, Marvin S and Kessler, Ronald C},
  journal={Behavioral sciences \& the law},
  volume={33},
  number={2-3},
  pages={199--212},
  year={2015},
  publisher={Wiley Online Library}
}

@article{simonyan2014very,
  title={Very deep convolutional networks for large-scale image recognition},
  author={Simonyan, Karen and Zisserman, Andrew},
  journal={arXiv preprint arXiv:1409.1556},
  year={2014}
}
@inproceedings{girshick2015fast,
  title={Fast r-cnn},
  author={Girshick, Ross},
  booktitle={Proceedings of the IEEE international conference on computer vision},
  pages={1440--1448},
  year={2015}
}
@inproceedings{bell2016inside,
  title={Inside-outside net: Detecting objects in context with skip pooling and recurrent neural networks},
  author={Bell, Sean and Lawrence Zitnick, C and Bala, Kavita and Girshick, Ross},
  booktitle={Proceedings of the IEEE conference on computer vision and pattern recognition},
  pages={2874--2883},
  year={2016}
}
@article{russakovsky2015imagenet,
  title={Imagenet large scale visual recognition challenge},
  author={Russakovsky, Olga and Deng, Jia and Su, Hao and Krause, Jonathan and Satheesh, Sanjeev and Ma, Sean and Huang, Zhiheng and Karpathy, Andrej and Khosla, Aditya and Bernstein, Michael and others},
  journal={International journal of computer vision},
  volume={115},
  number={3},
  pages={211--252},
  year={2015},
  publisher={Springer}
}
@inproceedings{lin2014microsoft,
  title={Microsoft coco: Common objects in context},
  author={Lin, Tsung-Yi and Maire, Michael and Belongie, Serge and Hays, James and Perona, Pietro and Ramanan, Deva and Doll{\'a}r, Piotr and Zitnick, C Lawrence},
  booktitle={European conference on computer vision},
  pages={740--755},
  year={2014},
  organization={Springer}
}
@article{everingham2007pascal,
  title={The PASCAL visual object classes challenge 2007 (VOC2007) results},
  author={Everingham, Mark and Van Gool, Luc and Williams, Christopher KI and Winn, John and Zisserman, Andrew},
  year={2007}
}
@inproceedings{zeiler2014visualizing,
  title={Visualizing and understanding convolutional networks},
  author={Zeiler, Matthew D and Fergus, Rob},
  booktitle={European conference on computer vision},
  pages={818--833},
  year={2014},
  organization={Springer}
}
@article{russakovsky2015imagenet,
  title={Imagenet large scale visual recognition challenge},
  author={Russakovsky, Olga and Deng, Jia and Su, Hao and Krause, Jonathan and Satheesh, Sanjeev and Ma, Sean and Huang, Zhiheng and Karpathy, Andrej and Khosla, Aditya and Bernstein, Michael and others},
  journal={International journal of computer vision},
  volume={115},
  number={3},
  pages={211--252},
  year={2015},
  publisher={Springer}
}

@inproceedings{park2000efficient,
  title={Efficient use of local edge histogram descriptor},
  author={Park, Dong Kwon and Jeon, Yoon Seok and Won, Chee Sun},
  booktitle={Proceedings of the 2000 ACM workshops on Multimedia},
  pages={51--54},
  year={2000},
  organization={ACM}
}
@article{ro2001mpeg,
  title={MPEG-7 homogeneous texture descriptor},
  author={Ro, Yong Man and Kim, Munchurl and Kang, Ho Kyung and Manjunath, BS and Kim, Jinwoong},
  journal={ETRI journal},
  volume={23},
  number={2},
  pages={41--51},
  year={2001},
  publisher={Wiley Online Library}
}
@article{malagon2009object,
  title={Object detection using image reconstruction with PCA},
  author={Malag{\'o}n-Borja, Luis and Fuentes, Olac},
  journal={Image and Vision Computing},
  volume={27},
  number={1-2},
  pages={2--9},
  year={2009},
  publisher={Elsevier}
}
@misc{knifedatabase,
  author = { Michał Grega},
  title = {{Knives Images Database}},
  howpublished = "\url{http://kt.agh.edu.pl/matiolanski/KnivesImagesDatabase/}",
  year = {2015}, 
  note = "[Online; accessed 25-November-2019]"
}
@misc{gunvideodatabase,
  author = {Grega},
  title = {{Guns movies database}},
  howpublished = "\url{http://kt.agh.edu.pl/grega/guns/}",
  year = {2013}, 
  note = "[Online; accessed 25-November-2019]"
}
@article{zawitz1995guns,
  title={Guns used in crime},
  author={Zawitz, Marianne W},
  journal={Washington, DC: US Department of Justice: Bureau of Justice Statistics Selected Findings, publication NCJ-148201},
  year={1995}
}

@article{lowe2004distinctive,
  title={Distinctive image features from scale-invariant keypoints},
  author={Lowe, David G},
  journal={International journal of computer vision},
  volume={60},
  number={2},
  pages={91--110},
  year={2004},
  publisher={Springer}
}

@misc{imfdb,
  author = {Evil Tim},
  title = {{The IMFDB Internet Movie Firearms Database}},
  howpublished = "\url{http://www.imfdb.org/wiki/Category:Gun}",
  year = {2011}, 
  note = "[Online; accessed 25-November-2019]"
}
@article{iqbal2019orientation,
  title={Orientation Aware Object Detection with Application to Firearms},
  author={Iqbal, Javed and Munir, Muhammad Akhtar and Mahmood, Arif and Ali, Afsheen Rafaqat and Ali, Mohsen},
  journal={arXiv preprint arXiv:1904.10032},
  year={2019}
}
@misc{shop,
  author = {Nick Enoch},
  title = {{Silver shop robbery goes wrong when customers fight back }},
  howpublished = "\url{https://www.dailymail.co.uk/news/article-4974230/Seville-shop-robbery-goes-wrong-customers-fight-back.html}",
  year = {2017}, 
  note = "[Online; accessed 08-August-2020]"
}
@misc{gunpoint,
  author = {Arif Nizami},
  title = {{Women escape armed robbery amid heavy traffic in DHA Lahore }},
  howpublished = "\url{https://www.pakistantoday.com.pk/2019/09/05/women-escape-armed-robbery-amid-heavy-traffic-in-dha/}",
  year = {2019}, 
  note = "[Online; accessed 08-August-2020]"
}
@misc{classification,
  author = {Arthur Ouaknine},
  title = {{Difference between Classification and Detection}},
  howpublished = "\url{https://medium.com/zylapp/review-of-deep-learning-algorithms-for-object-detection-c1f3d437b852}",
  year = {2018}, 
  note = "[Online; accessed 08-August-2020]"
}
@article{li2018multiscale,
  title={Multiscale rotated bounding Box-based deep learning method for detecting ship targets in remote sensing images},
  author={Li, Shuxin and Zhang, Zhilong and Li, Biao and Li, Chuwei},
  journal={Sensors},
  volume={18},
  number={8},
  pages={2702},
  year={2018},
  publisher={Multidisciplinary Digital Publishing Institute}
}
@article{liu2017learning,
  title={Learning a rotation invariant detector with rotatable bounding box},
  author={Liu, Lei and Pan, Zongxu and Lei, Bin},
  journal={arXiv preprint arXiv:1711.09405},
  year={2017}
}
@article{zagoruyko2016wide,
  title={Wide residual networks},
  author={Zagoruyko, Sergey and Komodakis, Nikos},
  journal={arXiv preprint arXiv:1605.07146},
  year={2016}
}

@inproceedings{nosaka2018orientation,
  title={Orientation-Aware Regression for Oriented Bounding Box Estimation},
  author={Nosaka, Ryusuke and Ujiie, Hidenori and Kurokawa, Takaharu},
  booktitle={2018 15th IEEE International Conference on Advanced Video and Signal Based Surveillance (AVSS)},
  pages={1--6},
  year={2018},
  organization={IEEE}
}
@inproceedings{ding2019learning,
  title={Learning RoI Transformer for Oriented Object Detection in Aerial Images},
  author={Ding, Jian and Xue, Nan and Long, Yang and Xia, Gui-Song and Lu, Qikai},
  booktitle={Proceedings of the IEEE Conference on Computer Vision and Pattern Recognition},
  pages={2849--2858},
  year={2019}
}
@inproceedings{xia2018dota,
  title={DOTA: A large-scale dataset for object detection in aerial images},
  author={Xia, Gui-Song and Bai, Xiang and Ding, Jian and Zhu, Zhen and Belongie, Serge and Luo, Jiebo and Datcu, Mihai and Pelillo, Marcello and Zhang, Liangpei},
  booktitle={Proceedings of the IEEE Conference on Computer Vision and Pattern Recognition},
  pages={3974--3983},
  year={2018}
}
@article{long2017accurate,
  title={Accurate object localization in remote sensing images based on convolutional neural networks},
  author={Long, Yang and Gong, Yiping and Xiao, Zhifeng and Liu, Qing},
  journal={IEEE Transactions on Geoscience and Remote Sensing},
  volume={55},
  number={5},
  pages={2486--2498},
  year={2017},
  publisher={IEEE}
}

@article{jiang2017r2cnn,
  title={R2cnn: Rotational region cnn for orientation robust scene text detection},
  author={Jiang, Yingying and Zhu, Xiangyu and Wang, Xiaobing and Yang, Shuli and Li, Wei and Wang, Hua and Fu, Pei and Luo, Zhenbo},
  journal={arXiv preprint arXiv:1706.09579},
  year={2017}
}

@inproceedings{szegedy2015going,
  title={Going deeper with convolutions},
  author={Szegedy, Christian and Liu, Wei and Jia, Yangqing and Sermanet, Pierre and Reed, Scott and Anguelov, Dragomir and Erhan, Dumitru and Vanhoucke, Vincent and Rabinovich, Andrew},
  booktitle={Proceedings of the IEEE conference on computer vision and pattern recognition},
  pages={1--9},
  year={2015}
}
@article{lenc2015r,
  title={R-cnn minus r},
  author={Lenc, Karel and Vedaldi, Andrea},
  journal={arXiv preprint arXiv:1506.06981},
  year={2015}
}
@inproceedings{yan2014fastest,
  title={The fastest deformable part model for object detection},
  author={Yan, Junjie and Lei, Zhen and Wen, Longyin and Li, Stan Z},
  booktitle={Proceedings of the IEEE Conference on Computer Vision and Pattern Recognition},
  pages={2497--2504},
  year={2014}
}
@misc{rolabelimg,
  author = {cgvict},
  title = {{roLabelImg}},
  howpublished = "\url{https://github.com/cgvict/roLabelImg}",
  year = {2017}, 
  note = "[Online; accessed 23-June-2020]"
}
@article{yang2019c,
  title={C-RPNs: Promoting object detection in real world via a cascade structure of Region Proposal Networks},
  author={Yang, Dongming and Zou, YueXian and Zhang, Jian and Li, Ge},
  journal={Neurocomputing},
  volume={367},
  pages={20--30},
  year={2019},
  publisher={Elsevier}
}
@article{gong2019using,
  title={Using multi-label classification to improve object detection},
  author={Gong, Tao and Liu, Bin and Chu, Qi and Yu, Nenghai},
  journal={neurocomputing},
  volume={370},
  pages={174--185},
  year={2019},
  publisher={Elsevier}
}
@article{wu2020recent,
  title={Recent advances in deep learning for object detection},
  author={Wu, Xiongwei and Sahoo, Doyen and Hoi, Steven CH},
  journal={Neurocomputing},
  year={2020},
  publisher={Elsevier}
}
@article{liu2016ship,
  title={Ship rotated bounding box space for ship extraction from high-resolution optical satellite images with complex backgrounds},
  author={Liu, Zikun and Wang, Hongzhen and Weng, Lubin and Yang, Yiping},
  journal={IEEE Geoscience and Remote Sensing Letters},
  volume={13},
  number={8},
  pages={1074--1078},
  year={2016},
  publisher={IEEE}
}

@article{kuznetsova2020open,
  title={The open images dataset v4},
  author={Kuznetsova, Alina and Rom, Hassan and Alldrin, Neil and Uijlings, Jasper and Krasin, Ivan and Pont-Tuset, Jordi and Kamali, Shahab and Popov, Stefan and Malloci, Matteo and Kolesnikov, Alexander and others},
  journal={International Journal of Computer Vision},
  pages={1--26},
  year={2020},
  publisher={Springer}
}
@inproceedings{fei2010imagenet,
  title={ImageNet: crowdsourcing, benchmarking \& other cool things},
  author={Fei-Fei, Li},
  booktitle={CMU VASC Seminar},
  volume={16},
  pages={18--25},
  year={2010}
}

@misc{gunsdataset,
  author = {S. Sasank},
  title = {{Guns Object Detection}},
  howpublished = "\url{https://www.kaggle.com/issaisasank/guns-object-detection}",
  year = {2019}, 
  note = "[Online; accessed 23-June-2020]"
}

